Integrated Balanced and Staggered Routing in Autonomous Mobility-on-Demand Systems

Autonomous mobility-on-demand (AMoD) systems, centrally coordinated fleets of self-driving vehicles, offer a promising alternative to traditional ride-hailing by improving traffic flow and reducing operating costs. Centralized control in AMoD systems enables two complementary routing strategies: balanced routing, which distributes traffic across alternative routes to ease congestion, and staggered routing, which delays departures to smooth peak demand over time. In this work, we introduce a unified framework that jointly optimizes both route choices and departure times to minimize system travel times. We formulate the problem as an optimization model and show that our congestion model yields an unbiased estimate of travel times derived from a discretized version of Vickrey's bottleneck model. To solve large-scale instances, we develop a custom metaheuristic based on a large neighborhood search framework. We assess our method through a case study on the Manhattan street network using real-world taxi data. In a setting with exclusively centrally controlled AMoD vehicles, our approach reduces total traffic delay by up to 25 percent and mitigates network congestion by up to 35 percent compared to selfish routing. We also consider mixed-traffic settings with both AMoD and conventional vehicles, comparing a welfare-oriented operator that minimizes total system travel time with a profit-oriented one that optimizes only the fleet's travel time. Independent of the operator's objective, the analysis reveals a win-win outcome: across all control levels, both autonomous and non-autonomous traffic benefit from the implementation of balancing and staggering strategies.

==> archive/bilevel_decomposition.tex <==
\subsection{Bilevel optimization formulation}
We model the joint route and departure-time assignment problem as a bilevel optimization problem. The upper level is responsible for assigning a single path to each trip, while the lower level determines the optimal departure times along the assigned paths to minimize delay under congestion. We define the binary variable $\ArcSelected{\Arc}{\Trip} \in \{0,1\}$ to indicate whether arc $\Arc$ is part of the selected route for trip $\Trip$. The free-flow travel time on arc $\Arc$ is given by $\NominalTravelTime{\Arc}$, while $\Delay{\Arc}{\Trip}$ denotes the congestion-induced delay experienced by trip $\Trip$ on arc $\Arc$. The decision variable $\Departure{\Arc}{\Trip}$ represents the start time of trip $\Trip$ on arc $\Arc$. 

To model congestion, we define $\Flow{\Arc}{\Trip}$ as the number of other trips using arc $\Arc$ and overlapping in time with trip $\Trip$. This value is used in a piecewise linear delay function parameterized by $(\mu^k_a, \ThFlow{\Arc}{k})$ for $k = 1, \dots, K$. For each node $i \in \Nodes$, let $\Ingoing{i}$ and $\Outgoing{i}$ denote the sets of arcs entering and leaving node $i$, respectively. The successor of an arc on a selected route is denoted by $\Successor{\Arc}$. Finally, $M$ is a sufficiently large constant used in big-M formulations.

\subsection{Upper-Level Problem: Route Assignment}

The upper level chooses a path for each trip by selecting arcs that form a valid origin-destination route. The objective is to minimize total travel time, consisting of both free-flow and congestion-related delays as returned by the lower level.

\begin{align}
\min_{\ArcSelection} \quad \Phi\left(\ArcSelection, \OptimalDelays\right) 
&:= \textstyle\sum_{\Trip \in \SetTrips} \sum_{\Arc \in \Arcs} (\NominalTravelTime{\Arc} + \OptimalDelay{\Trip}{\Arc}) \cdot \ArcSelected{\Arc}{\Trip} \quad &\label{eq:upper_obj} \\
\text{s.t.} \quad 
\textstyle\sum_{\Arc \in \Outgoing{\Origin{\Trip}}} \ArcSelected{\Arc}{\Trip} 
&= 1 
\quad && \forall \Trip \in \SetTrips \quad &\label{eq:flow_origin} \\
\textstyle\sum_{\Arc \in \Ingoing{\Destination{\Trip}}} \ArcSelected{\Arc}{\Trip} 
&= 1 
\quad && \forall \Trip \in \SetTrips \quad &\label{eq:flow_dest} \\
\textstyle\sum_{\Arc \in \Outgoing{i}} \ArcSelected{\Arc}{\Trip} - \sum_{\Arc \in \Ingoing{i}} \ArcSelected{\Arc}{\Trip} 
&= 0 
\quad && \forall \Trip \in \SetTrips, \; \forall i \in \Nodes \setminus \{\Origin{\Trip}, \Destination{\Trip}\} \quad &\label{eq:flow_balance} \\
\ArcSelected{\Arc}{\Trip} 
&\in \{0, 1\} 
\quad && \forall \Trip \in \SetTrips,\; \Arc \in \Arcs \quad &\label{eq:binary_constraint} \\
\OptimalDelays 
&\in \arg\min_{x} \LowerLevel 
\quad && \quad &\label{eq:lower_link}
\end{align}

Constraints~\eqref{eq:flow_origin}--\eqref{eq:flow_balance} enforce flow conservation, ensuring that each trip is assigned a valid $s$-$t$ path. Constraint~\eqref{eq:binary_constraint} defines arc inclusion decisions as binary variables. The coupling constraint~\eqref{eq:lower_link} links the upper and lower levels, requiring that delays are computed as the solution of the lower-level problem.

\subsection{Lower-Level Problem: Departure Time Optimization under Congestion}

Given a set of selected routes, the lower-level problem schedules the departure times and evaluates delays along those routes, accounting for congestion through temporal overlap.

\begin{alignat}{4}
\min_{x} \quad \LowerLevel 
&:= \textstyle\sum_{\Trip \in \SetTrips} \sum_{\Arc \in \Arcs} \Delay{\Arc}{\Trip}
\quad && \label{eq:lower_obj} \\
\text{s.t.} \quad 
\Delay{\Arc}{\Trip} 
&\ge \textstyle\sum_{k = 1}^{K} \mu^k_a (\Flow{\Arc}{\Trip} - \ThFlow{\Arc}{k}) 
\quad && \forall \Trip \in \SetTrips, \Arc \in \Arcs \quad &\label{eq:delay_def} \\
\Departure{\Successor{\Arc}}{\Trip} 
&= \Departure{\Arc}{\Trip} + \NominalTravelTime{\Arc} + \Delay{\Arc}{\Trip} 
\quad && \forall \Trip \in \SetTrips, \Arc \in \Arcs \setminus \{\Destination{\Trip}\} \quad &\label{eq:time_prop} \\
\Flow{\Arc}{\Trip} 
&= \textstyle\sum_{\SecondTrip \ne \Trip} 
\mathbb{I}\left(
\Departure{\Arc}{\SecondTrip} \le \Departure{\Arc}{\Trip} < \Departure{\Successor{\Arc}}{\SecondTrip}
\right) \cdot \ArcSelected{\Arc}{\SecondTrip} \cdot \ArcSelected{\Arc}{\Trip} 
\quad && \forall \Trip \in \SetTrips, \Arc \in \Arcs \quad &\label{eq:overlap} \\
\TripEarliestDeparture{\Trip} 
&\le \textstyle\Departure{\Arc}{\Trip} \le \TripEarliestDeparture{\Trip} + \TripMaxStaggering{\Trip} 
\quad && \forall \Trip \in \SetTrips,\; \forall \Arc \in \Outgoing{\Origin{\Trip}} \quad &\label{eq:staggering_window} \\
\Departure{\Arc}{\Trip} + \NominalTravelTime{\Arc} + \Delay{\Arc}{\Trip} 
&\le \TripLatestArrival{\Trip} 
\quad && \forall \Trip \in \SetTrips,\; \forall \Arc \in \Ingoing{\Destination{\Trip}} \quad &\label{eq:arrival_deadline} \\
\Delay{\Arc}{\Trip},\; \Departure{\Arc}{\Trip},\; \Flow{\Arc}{\Trip} 
&\ge 0 
\quad && \forall \Trip \in \SetTrips, \Arc \in \Arcs \quad &\label{eq:nonnegativity}
\end{alignat}

The objective in~\eqref{eq:lower_obj} minimizes the total delay experienced by all trips on the network. Constraint~\eqref{eq:delay_def} models the delay as a piecewise linear function of congestion. Constraint~\eqref{eq:time_prop} propagates departure times along the route. Constraint~\eqref{eq:overlap} defines arc congestion as the count of overlapping trips, and ensures that flow variables are zero on non-selected arcs due to the multiplicative structure involving \(\ArcSelected{\Arc}{\Trip}\). As a result, the delay variables associated with unused arcs are not penalized in the objective and are naturally driven to zero. Constraint~\eqref{eq:staggering_window} enforces that the departure occurs within an allowable time window, while~\eqref{eq:arrival_deadline} guarantees that trips arrive before their latest permissible arrival times. Finally, Constraint~\eqref{eq:nonnegativity} enforces non-negativity of delay, departure time, and congestion variables.

\subsection{Compact Single-Level Reformulation}

We reformulate the bilevel model as a single-level optimization problem by explicitly embedding the departure time and delay optimization within the route assignment model. The resulting formulation jointly determines the route and departure time of each trip while accounting for congestion through temporal overlap on shared arcs.

\begin{alignat}{4}
\min \quad 
& \textstyle\sum_{\Trip \in \SetTrips} \sum_{\Arc \in \Arcs} (\NominalTravelTime{\Arc} \cdot \ArcSelected{\Arc}{\Trip} + \Delay{\Arc}{\Trip}) 
\quad && \label{eq:single_obj} \\
\text{s.t.} \quad 
& \textstyle\sum_{\Arc \in \Outgoing{\Origin{\Trip}}} \ArcSelected{\Arc}{\Trip} = 1 
\quad && \forall \Trip \in \SetTrips \quad &\label{eq:single_origin} \\
& \textstyle\sum_{\Arc \in \Ingoing{\Destination{\Trip}}} \ArcSelected{\Arc}{\Trip} = 1 
\quad && \forall \Trip \in \SetTrips \quad &\label{eq:single_dest} \\
& \textstyle\sum_{\Arc \in \Outgoing{i}} \ArcSelected{\Arc}{\Trip} - \sum_{\Arc \in \Ingoing{i}} \ArcSelected{\Arc}{\Trip} = 0 
\quad && \forall \Trip \in \SetTrips,\; \forall i \in \Nodes \setminus \{\Origin{\Trip}, \Destination{\Trip}\} \quad &\label{eq:single_balance} \\
& \Delay{\Arc}{\Trip} 
\ge \textstyle\sum_{k = 1}^{K} \mu^k_a (\Flow{\Arc}{\Trip} - \ThFlow{\Arc}{k}) 
\quad && \forall \Trip, \Arc \quad &\label{eq:single_delay} \\
& \Departure{\Successor{\Arc}}{\Trip} 
= \Departure{\Arc}{\Trip} + \NominalTravelTime{\Arc} + \Delay{\Arc}{\Trip} 
\quad && \forall \Trip \in \SetTrips,\; \Arc \in \Arcs \quad &\label{eq:single_propagation} \\
& \Flow{\Arc}{\Trip} 
= \textstyle\sum_{\SecondTrip \ne \Trip} 
\mathbb{I}\left(
\Departure{\Arc}{\SecondTrip} \le \Departure{\Arc}{\Trip} < \Departure{\Successor{\Arc}}{\SecondTrip}
\right) \cdot \ArcSelected{\Arc}{\SecondTrip} \cdot \ArcSelected{\Arc}{\Trip} 
\quad && \forall \Trip, \Arc \quad &\label{eq:single_overlap} \\
& \TripEarliestDeparture{\Trip} 
\le \Departure{\Arc}{\Trip} 
\le \TripEarliestDeparture{\Trip} + \TripMaxStaggering{\Trip}
\quad && \forall \Trip,\; \Arc \in \Outgoing{\Origin{\Trip}} \quad &\label{eq:single_staggering} \\
& \Departure{\Arc}{\Trip} + \NominalTravelTime{\Arc} + \Delay{\Arc}{\Trip} 
\le \TripLatestArrival{\Trip} 
\quad && \forall \Trip,\; \Arc \in \Ingoing{\Destination{\Trip}} \quad &\label{eq:single_arrival} \\
& \Delay{\Arc}{\Trip},\; \Departure{\Arc}{\Trip},\; \Flow{\Arc}{\Trip} \ge 0 
\quad && \forall \Trip, \Arc \in \Arcs \quad &\label{eq:single_nonneg} \\
& \ArcSelected{\Arc}{\Trip} \in \{0,1\} 
\quad && \forall \Trip \in \SetTrips,\; \Arc \in \Arcs \quad &\label{eq:single_binary}
\end{alignat}

Constraints~\eqref{eq:single_origin}--\eqref{eq:single_balance} define valid paths for each trip. Delay and congestion are modeled in~\eqref{eq:single_delay} and~\eqref{eq:single_overlap}. Time propagation is enforced in~\eqref{eq:single_propagation}, and feasibility of departure and arrival times is guaranteed by~\eqref{eq:single_staggering}--\eqref{eq:single_arrival}. Constraints~\eqref{eq:single_nonneg} and~\eqref{eq:single_binary} define variable domains.
Although the delay variables $\Delay{\Arc}{\Trip}$ are not multiplied by the binary selection variable $\ArcSelected{\Arc}{\Trip}$ in the objective~\eqref{eq:single_obj}, they are naturally driven to zero for non-selected arcs due to the congestion structure in~\eqref{eq:single_overlap} and the minimization direction. Therefore, the objective remains linear and correctly accounts only for delays incurred along the selected route.

==> figures/experiments/alternative_paths_comparison/boxplot_vary_theta.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray162159194}{RGB}{162,159,194}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{dimgray86}{RGB}{86,86,86}
\definecolor{lavender233232240}{RGB}{233,232,240}
\definecolor{lightgray201201221}{RGB}{201,201,221}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightslategray126118169}{RGB}{126,118,169}

\begin{axis}[height=\RouteFigureHeight,width=\RouteFigureWidth,
legend cell align={left},
legend style={
  fill opacity=1,
  draw opacity=1,
  text opacity=1,
  at={(1.01,1)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$\theta$},
xmajorgrids,
xmin=-0.5, xmax=4.5,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={0.0,0.2,0.4,0.6,0.8},
y grid style={darkgray176},
ylabel={[hrs]},
ymajorgrids,
ymin=5, ymax=50,
ytick style={color=black}
]
\addlegendimage{empty legend}
\addlegendentry{\hspace{-0.5cm} $k$}
\draw[draw=dimgray86,fill=lavender233232240,thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{mark=square*,draw=dimgray86,fill=lavender233232240,thick}
\addlegendentry{5}

\draw[draw=dimgray86,fill=lightgray201201221,thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{mark=square*,draw=dimgray86,fill=lightgray201201221,thick}
\addlegendentry{10}

\draw[draw=dimgray86,fill=darkgray162159194,thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{mark=square*,draw=dimgray86,fill=darkgray162159194,thick}
\addlegendentry{20}

\draw[draw=dimgray86,fill=lightslategray126118169,thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{mark=square*,draw=dimgray86,fill=lightslategray126118169,thick}
\addlegendentry{30}

\addplot [thick, dimgray86, forget plot]
table {%
-0.1875 23.3423840833333
-0.1875 15.3074101388889
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.1875 33.5771875555556
-0.1875 46.9209156111111
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.21875 15.3074101388889
-0.15625 15.3074101388889
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.21875 46.9209156111111
-0.15625 46.9209156111111
};
\addplot [thick, dimgray86, forget plot]
table {%
0.8125 18.21424525
0.8125 12.9437625277778
};
\addplot [thick, dimgray86, forget plot]
table {%
0.8125 24.5229223055556
0.8125 31.6245498611111
};
\addplot [thick, dimgray86, forget plot]
table {%
0.78125 12.9437625277778
0.84375 12.9437625277778
};
\addplot [thick, dimgray86, forget plot]
table {%
0.78125 31.6245498611111
0.84375 31.6245498611111
};
\addplot [thick, dimgray86, forget plot]
table {%
1.8125 15.8716713055556
1.8125 11.3482475277778
};
\addplot [thick, dimgray86, forget plot]
table {%
1.8125 21.3030847083333
1.8125 29.4093228611111
};
\addplot [thick, dimgray86, forget plot]
table {%
1.78125 11.3482475277778
1.84375 11.3482475277778
};
\addplot [thick, dimgray86, forget plot]
table {%
1.78125 29.4093228611111
1.84375 29.4093228611111
};
\addplot [thick, dimgray86, forget plot]
table {%
2.8125 14.3331522916667
2.8125 10.4621043888889
};
\addplot [thick, dimgray86, forget plot]
table {%
2.8125 19.3342388333333
2.8125 24.6960638055556
};
\addplot [thick, dimgray86, forget plot]
table {%
2.78125 10.4621043888889
2.84375 10.4621043888889
};
\addplot [thick, dimgray86, forget plot]
table {%
2.78125 24.6960638055556
2.84375 24.6960638055556
};
\addplot [thick, dimgray86, forget plot]
table {%
3.8125 14.163575
3.8125 10.6097008888889
};
\addplot [thick, dimgray86, forget plot]
table {%
3.8125 20.2148954027778
3.8125 25.9507678333333
};
\addplot [thick, dimgray86, forget plot]
table {%
3.78125 10.6097008888889
3.84375 10.6097008888889
};
\addplot [thick, dimgray86, forget plot]
table {%
3.78125 25.9507678333333
3.84375 25.9507678333333
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.0625 23.3423840833333
-0.0625 15.3074101388889
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.0625 33.5771875555556
-0.0625 46.9209156111111
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.09375 15.3074101388889
-0.03125 15.3074101388889
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.09375 46.9209156111111
-0.03125 46.9209156111111
};
\addplot [thick, dimgray86, forget plot]
table {%
0.9375 18.21424525
0.9375 12.9437625277778
};
\addplot [thick, dimgray86, forget plot]
table {%
0.9375 24.5229223055556
0.9375 31.6245498611111
};
\addplot [thick, dimgray86, forget plot]
table {%
0.90625 12.9437625277778
0.96875 12.9437625277778
};
\addplot [thick, dimgray86, forget plot]
table {%
0.90625 31.6245498611111
0.96875 31.6245498611111
};
\addplot [thick, dimgray86, forget plot]
table {%
1.9375 15.8716713055556
1.9375 11.3482475277778
};
\addplot [thick, dimgray86, forget plot]
table {%
1.9375 21.3030847083333
1.9375 26.8161226111111
};
\addplot [thick, dimgray86, forget plot]
table {%
1.90625 11.3482475277778
1.96875 11.3482475277778
};
\addplot [thick, dimgray86, forget plot]
table {%
1.90625 26.8161226111111
1.96875 26.8161226111111
};
\addplot [thick, dimgray86, forget plot]
table {%
2.9375 14.2005351666667
2.9375 10.4769478611111
};
\addplot [thick, dimgray86, forget plot]
table {%
2.9375 19.2317042222222
2.9375 24.4262883611111
};
\addplot [thick, dimgray86, forget plot]
table {%
2.90625 10.4769478611111
2.96875 10.4769478611111
};
\addplot [thick, dimgray86, forget plot]
table {%
2.90625 24.4262883611111
2.96875 24.4262883611111
};
\addplot [thick, dimgray86, forget plot]
table {%
3.9375 13.3291713611111
3.9375 9.82705275
};
\addplot [thick, dimgray86, forget plot]
table {%
3.9375 18.1357970694444
3.9375 25.2494230555556
};
\addplot [thick, dimgray86, forget plot]
table {%
3.90625 9.82705275
3.96875 9.82705275
};
\addplot [thick, dimgray86, forget plot]
table {%
3.90625 25.2494230555556
3.96875 25.2494230555556
};
\addplot [thick, dimgray86, forget plot]
table {%
0.0625 23.3423840833333
0.0625 15.3074101388889
};
\addplot [thick, dimgray86, forget plot]
table {%
0.0625 33.5771875555556
0.0625 46.9209156111111
};
\addplot [thick, dimgray86, forget plot]
table {%
0.03125 15.3074101388889
0.09375 15.3074101388889
};
\addplot [thick, dimgray86, forget plot]
table {%
0.03125 46.9209156111111
0.09375 46.9209156111111
};
\addplot [thick, dimgray86, forget plot]
table {%
1.0625 18.21424525
1.0625 12.9437625277778
};
\addplot [thick, dimgray86, forget plot]
table {%
1.0625 24.5229223055556
1.0625 31.6245498611111
};
\addplot [thick, dimgray86, forget plot]
table {%
1.03125 12.9437625277778
1.09375 12.9437625277778
};
\addplot [thick, dimgray86, forget plot]
table {%
1.03125 31.6245498611111
1.09375 31.6245498611111
};
\addplot [thick, dimgray86, forget plot]
table {%
2.0625 15.8716713055556
2.0625 11.3482475277778
};
\addplot [thick, dimgray86, forget plot]
table {%
2.0625 21.3030847083333
2.0625 26.8161226111111
};
\addplot [thick, dimgray86, forget plot]
table {%
2.03125 11.3482475277778
2.09375 11.3482475277778
};
\addplot [thick, dimgray86, forget plot]
table {%
2.03125 26.8161226111111
2.09375 26.8161226111111
};
\addplot [thick, dimgray86, forget plot]
table {%
3.0625 14.2005351666667
3.0625 10.4769478611111
};
\addplot [thick, dimgray86, forget plot]
table {%
3.0625 19.2317042222222
3.0625 24.8505323888889
};
\addplot [thick, dimgray86, forget plot]
table {%
3.03125 10.4769478611111
3.09375 10.4769478611111
};
\addplot [thick, dimgray86, forget plot]
table {%
3.03125 24.8505323888889
3.09375 24.8505323888889
};
\addplot [thick, dimgray86, forget plot]
table {%
4.0625 13.2250305416667
4.0625 9.87289869444444
};
\addplot [thick, dimgray86, forget plot]
table {%
4.0625 17.9955574444444
4.0625 24.6023948611111
};
\addplot [thick, dimgray86, forget plot]
table {%
4.03125 9.87289869444444
4.09375 9.87289869444444
};
\addplot [thick, dimgray86, forget plot]
table {%
4.03125 24.6023948611111
4.09375 24.6023948611111
};
\addplot [thick, dimgray86, forget plot]
table {%
0.1875 23.3423840833333
0.1875 15.3074101388889
};
\addplot [thick, dimgray86, forget plot]
table {%
0.1875 33.5771875555556
0.1875 46.9209156111111
};
\addplot [thick, dimgray86, forget plot]
table {%
0.15625 15.3074101388889
0.21875 15.3074101388889
};
\addplot [thick, dimgray86, forget plot]
table {%
0.15625 46.9209156111111
0.21875 46.9209156111111
};
\addplot [thick, dimgray86, forget plot]
table {%
1.1875 18.21424525
1.1875 12.9437625277778
};
\addplot [thick, dimgray86, forget plot]
table {%
1.1875 24.5229223055556
1.1875 31.6245498611111
};
\addplot [thick, dimgray86, forget plot]
table {%
1.15625 12.9437625277778
1.21875 12.9437625277778
};
\addplot [thick, dimgray86, forget plot]
table {%
1.15625 31.6245498611111
1.21875 31.6245498611111
};
\addplot [thick, dimgray86, forget plot]
table {%
2.1875 15.8716713055556
2.1875 11.3482475277778
};
\addplot [thick, dimgray86, forget plot]
table {%
2.1875 21.3030847083333
2.1875 26.8161226111111
};
\addplot [thick, dimgray86, forget plot]
table {%
2.15625 11.3482475277778
2.21875 11.3482475277778
};
\addplot [thick, dimgray86, forget plot]
table {%
2.15625 26.8161226111111
2.21875 26.8161226111111
};
\addplot [thick, dimgray86, forget plot]
table {%
3.1875 14.2005351666667
3.1875 10.4769478611111
};
\addplot [thick, dimgray86, forget plot]
table {%
3.1875 19.2317042222222
3.1875 24.8505323888889
};
\addplot [thick, dimgray86, forget plot]
table {%
3.15625 10.4769478611111
3.21875 10.4769478611111
};
\addplot [thick, dimgray86, forget plot]
table {%
3.15625 24.8505323888889
3.21875 24.8505323888889
};
\addplot [thick, dimgray86, forget plot]
table {%
4.1875 13.3622424583333
4.1875 9.89431819444444
};
\addplot [thick, dimgray86, forget plot]
table {%
4.1875 17.8190193472222
4.1875 24.4444096111111
};
\addplot [thick, dimgray86, forget plot]
table {%
4.15625 9.89431819444444
4.21875 9.89431819444444
};
\addplot [thick, dimgray86, forget plot]
table {%
4.15625 24.4444096111111
4.21875 24.4444096111111
};
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:-0.25,23.3423840833333)
--(axis cs:-0.125,23.3423840833333)
--(axis cs:-0.125,33.5771875555556)
--(axis cs:-0.25,33.5771875555556)
--(axis cs:-0.25,23.3423840833333)
--cycle;
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:0.75,18.21424525)
--(axis cs:0.875,18.21424525)
--(axis cs:0.875,24.5229223055556)
--(axis cs:0.75,24.5229223055556)
--(axis cs:0.75,18.21424525)
--cycle;
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:1.75,15.8716713055556)
--(axis cs:1.875,15.8716713055556)
--(axis cs:1.875,21.3030847083333)
--(axis cs:1.75,21.3030847083333)
--(axis cs:1.75,15.8716713055556)
--cycle;
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:2.75,14.3331522916667)
--(axis cs:2.875,14.3331522916667)
--(axis cs:2.875,19.3342388333333)
--(axis cs:2.75,19.3342388333333)
--(axis cs:2.75,14.3331522916667)
--cycle;
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:3.75,14.163575)
--(axis cs:3.875,14.163575)
--(axis cs:3.875,20.2148954027778)
--(axis cs:3.75,20.2148954027778)
--(axis cs:3.75,14.163575)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:-0.125,23.3423840833333)
--(axis cs:0,23.3423840833333)
--(axis cs:0,33.5771875555556)
--(axis cs:-0.125,33.5771875555556)
--(axis cs:-0.125,23.3423840833333)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:0.875,18.21424525)
--(axis cs:1,18.21424525)
--(axis cs:1,24.5229223055556)
--(axis cs:0.875,24.5229223055556)
--(axis cs:0.875,18.21424525)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:1.875,15.8716713055556)
--(axis cs:2,15.8716713055556)
--(axis cs:2,21.3030847083333)
--(axis cs:1.875,21.3030847083333)
--(axis cs:1.875,15.8716713055556)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:2.875,14.2005351666667)
--(axis cs:3,14.2005351666667)
--(axis cs:3,19.2317042222222)
--(axis cs:2.875,19.2317042222222)
--(axis cs:2.875,14.2005351666667)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:3.875,13.3291713611111)
--(axis cs:4,13.3291713611111)
--(axis cs:4,18.1357970694444)
--(axis cs:3.875,18.1357970694444)
--(axis cs:3.875,13.3291713611111)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:0,23.3423840833333)
--(axis cs:0.125,23.3423840833333)
--(axis cs:0.125,33.5771875555556)
--(axis cs:0,33.5771875555556)
--(axis cs:0,23.3423840833333)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:1,18.21424525)
--(axis cs:1.125,18.21424525)
--(axis cs:1.125,24.5229223055556)
--(axis cs:1,24.5229223055556)
--(axis cs:1,18.21424525)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:2,15.8716713055556)
--(axis cs:2.125,15.8716713055556)
--(axis cs:2.125,21.3030847083333)
--(axis cs:2,21.3030847083333)
--(axis cs:2,15.8716713055556)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:3,14.2005351666667)
--(axis cs:3.125,14.2005351666667)
--(axis cs:3.125,19.2317042222222)
--(axis cs:3,19.2317042222222)
--(axis cs:3,14.2005351666667)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:4,13.2250305416667)
--(axis cs:4.125,13.2250305416667)
--(axis cs:4.125,17.9955574444444)
--(axis cs:4,17.9955574444444)
--(axis cs:4,13.2250305416667)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:0.125,23.3423840833333)
--(axis cs:0.25,23.3423840833333)
--(axis cs:0.25,33.5771875555556)
--(axis cs:0.125,33.5771875555556)
--(axis cs:0.125,23.3423840833333)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:1.125,18.21424525)
--(axis cs:1.25,18.21424525)
--(axis cs:1.25,24.5229223055556)
--(axis cs:1.125,24.5229223055556)
--(axis cs:1.125,18.21424525)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:2.125,15.8716713055556)
--(axis cs:2.25,15.8716713055556)
--(axis cs:2.25,21.3030847083333)
--(axis cs:2.125,21.3030847083333)
--(axis cs:2.125,15.8716713055556)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:3.125,14.2005351666667)
--(axis cs:3.25,14.2005351666667)
--(axis cs:3.25,19.2317042222222)
--(axis cs:3.125,19.2317042222222)
--(axis cs:3.125,14.2005351666667)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:4.125,13.3622424583333)
--(axis cs:4.25,13.3622424583333)
--(axis cs:4.25,17.8190193472222)
--(axis cs:4.125,17.8190193472222)
--(axis cs:4.125,13.3622424583333)
--cycle;
\addplot [thick, dimgray86, forget plot]
table {%
-0.25 26.7689764444444
-0.125 26.7689764444444
};
\addplot [thick, dimgray86, forget plot]
table {%
0.75 20.6129742222222
0.875 20.6129742222222
};
\addplot [thick, dimgray86, forget plot]
table {%
1.75 18.30105175
1.875 18.30105175
};
\addplot [thick, dimgray86, forget plot]
table {%
2.75 16.7342374722222
2.875 16.7342374722222
};
\addplot [thick, dimgray86, forget plot]
table {%
3.75 16.734838
3.875 16.734838
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.125 26.7689764444444
0 26.7689764444444
};
\addplot [thick, dimgray86, forget plot]
table {%
0.875 20.6129742222222
1 20.6129742222222
};
\addplot [thick, dimgray86, forget plot]
table {%
1.875 18.30105175
2 18.30105175
};
\addplot [thick, dimgray86, forget plot]
table {%
2.875 16.5567049722222
3 16.5567049722222
};
\addplot [thick, dimgray86, forget plot]
table {%
3.875 15.4163099166667
4 15.4163099166667
};
\addplot [thick, dimgray86, forget plot]
table {%
0 26.7689764444444
0.125 26.7689764444444
};
\addplot [thick, dimgray86, forget plot]
table {%
1 20.6129742222222
1.125 20.6129742222222
};
\addplot [thick, dimgray86, forget plot]
table {%
2 18.30105175
2.125 18.30105175
};
\addplot [thick, dimgray86, forget plot]
table {%
3 16.5567049722222
3.125 16.5567049722222
};
\addplot [thick, dimgray86, forget plot]
table {%
4 15.7262033611111
4.125 15.7262033611111
};
\addplot [thick, dimgray86, forget plot]
table {%
0.125 26.7689764444444
0.25 26.7689764444444
};
\addplot [thick, dimgray86, forget plot]
table {%
1.125 20.6129742222222
1.25 20.6129742222222
};
\addplot [thick, dimgray86, forget plot]
table {%
2.125 18.30105175
2.25 18.30105175
};
\addplot [thick, dimgray86, forget plot]
table {%
3.125 16.5567049722222
3.25 16.5567049722222
};
\addplot [thick, dimgray86, forget plot]
table {%
4.125 15.3065178611111
4.25 15.3065178611111
};
\end{axis}

\end{tikzpicture}


==> figures/experiments/alternative_paths_comparison/boxplot_vary_theta_runtimes.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray162159194}{RGB}{162,159,194}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{dimgray86}{RGB}{86,86,86}
\definecolor{lavender233232240}{RGB}{233,232,240}
\definecolor{lightgray201201221}{RGB}{201,201,221}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightslategray126118169}{RGB}{126,118,169}

\begin{axis}[height=\RouteFigureHeight,width=\RouteFigureWidth,
legend cell align={left},
legend style={
  fill opacity=1,
  draw opacity=1,
  text opacity=1,
  at={(1.01,1)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$\theta$},
xmajorgrids,
xmin=-0.5, xmax=4.5,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={0.0,0.2,0.4,0.6,0.8},
y grid style={darkgray176},
ylabel={[min]},
ymajorgrids,
ymin=0, ymax=5,
ytick style={color=black}
]
\addlegendimage{empty legend}
\addlegendentry{\hspace{-0.5cm} $k$}
\draw[draw=dimgray86,fill=lavender233232240,thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{mark=square*,draw=dimgray86,fill=lavender233232240,thick}
\addlegendentry{5}

\draw[draw=dimgray86,fill=lightgray201201221,thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{mark=square*,draw=dimgray86,fill=lightgray201201221,thick}
\addlegendentry{10}

\draw[draw=dimgray86,fill=darkgray162159194,thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{mark=square*,draw=dimgray86,fill=darkgray162159194,thick}
\addlegendentry{20}

\draw[draw=dimgray86,fill=lightslategray126118169,thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{mark=square*,draw=dimgray86,fill=lightslategray126118169,thick}
\addlegendentry{30}

\addplot [thick, dimgray86, forget plot]
table {%
-0.1875 0.0868333333333333
-0.1875 0.0303333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.1875 0.2115
-0.1875 0.299
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.21875 0.0303333333333333
-0.15625 0.0303333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.21875 0.299
-0.15625 0.299
};
\addplot [thick, dimgray86, forget plot]
table {%
0.8125 0.147583333333333
0.8125 0.0333333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
0.8125 0.272583333333333
0.8125 0.296166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
0.78125 0.0333333333333333
0.84375 0.0333333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
0.78125 0.296166666666667
0.84375 0.296166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
1.8125 0.127833333333333
1.8125 0.0531666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
1.8125 0.334583333333333
1.8125 0.634333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
1.78125 0.0531666666666667
1.84375 0.0531666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
1.78125 0.634333333333333
1.84375 0.634333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
2.8125 0.31325
2.8125 0.0798333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
2.8125 0.869
2.8125 1.104
};
\addplot [thick, dimgray86, forget plot]
table {%
2.78125 0.0798333333333333
2.84375 0.0798333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
2.78125 1.104
2.84375 1.104
};
\addplot [thick, dimgray86, forget plot]
table {%
3.8125 0.35675
3.8125 0.152
};
\addplot [thick, dimgray86, forget plot]
table {%
3.8125 0.869833333333333
3.8125 0.874
};
\addplot [thick, dimgray86, forget plot]
table {%
3.78125 0.152
3.84375 0.152
};
\addplot [thick, dimgray86, forget plot]
table {%
3.78125 0.874
3.84375 0.874
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.0625 0.0768333333333333
-0.0625 0.033
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.0625 0.266083333333333
-0.0625 0.373166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.09375 0.033
-0.03125 0.033
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.09375 0.373166666666667
-0.03125 0.373166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
0.9375 0.126
0.9375 0.0856666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
0.9375 0.265166666666667
0.9375 0.292
};
\addplot [thick, dimgray86, forget plot]
table {%
0.90625 0.0856666666666667
0.96875 0.0856666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
0.90625 0.292
0.96875 0.292
};
\addplot [thick, dimgray86, forget plot]
table {%
1.9375 0.120083333333333
1.9375 0.0686666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
1.9375 0.3015
1.9375 0.3055
};
\addplot [thick, dimgray86, forget plot]
table {%
1.90625 0.0686666666666667
1.96875 0.0686666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
1.90625 0.3055
1.96875 0.3055
};
\addplot [thick, dimgray86, forget plot]
table {%
2.9375 0.297
2.9375 0.110166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
2.9375 0.640333333333333
2.9375 1.07716666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
2.90625 0.110166666666667
2.96875 0.110166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
2.90625 1.07716666666667
2.96875 1.07716666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
3.9375 0.403916666666667
3.9375 0.288333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
3.9375 1.15016666666667
3.9375 2.10233333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
3.90625 0.288333333333333
3.96875 0.288333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
3.90625 2.10233333333333
3.96875 2.10233333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
0.0625 0.0659166666666667
0.0625 0.021
};
\addplot [thick, dimgray86, forget plot]
table {%
0.0625 0.218666666666667
0.0625 0.221666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
0.03125 0.021
0.09375 0.021
};
\addplot [thick, dimgray86, forget plot]
table {%
0.03125 0.221666666666667
0.09375 0.221666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
1.0625 0.107333333333333
1.0625 0.0665
};
\addplot [thick, dimgray86, forget plot]
table {%
1.0625 0.225
1.0625 0.253
};
\addplot [thick, dimgray86, forget plot]
table {%
1.03125 0.0665
1.09375 0.0665
};
\addplot [thick, dimgray86, forget plot]
table {%
1.03125 0.253
1.09375 0.253
};
\addplot [thick, dimgray86, forget plot]
table {%
2.0625 0.148
2.0625 0.0673333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
2.0625 0.311416666666667
2.0625 0.345666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
2.03125 0.0673333333333333
2.09375 0.0673333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
2.03125 0.345666666666667
2.09375 0.345666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
3.0625 0.24525
3.0625 0.161333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
3.0625 0.5255
3.0625 0.556833333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
3.03125 0.161333333333333
3.09375 0.161333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
3.03125 0.556833333333333
3.09375 0.556833333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
4.0625 0.47625
4.0625 0.224166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
4.0625 2.01225
4.0625 3.143
};
\addplot [thick, dimgray86, forget plot]
table {%
4.03125 0.224166666666667
4.09375 0.224166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
4.03125 3.143
4.09375 3.143
};
\addplot [thick, dimgray86, forget plot]
table {%
0.1875 0.0585
0.1875 0.0466666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
0.1875 0.225
0.1875 0.267
};
\addplot [thick, dimgray86, forget plot]
table {%
0.15625 0.0466666666666667
0.21875 0.0466666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
0.15625 0.267
0.21875 0.267
};
\addplot [thick, dimgray86, forget plot]
table {%
1.1875 0.0981666666666667
1.1875 0.043
};
\addplot [thick, dimgray86, forget plot]
table {%
1.1875 0.191083333333333
1.1875 0.202666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
1.15625 0.043
1.21875 0.043
};
\addplot [thick, dimgray86, forget plot]
table {%
1.15625 0.202666666666667
1.21875 0.202666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
2.1875 0.146916666666667
2.1875 0.0863333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
2.1875 0.306916666666667
2.1875 0.316166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
2.15625 0.0863333333333333
2.21875 0.0863333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
2.15625 0.316166666666667
2.21875 0.316166666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
3.1875 0.240083333333333
3.1875 0.0921666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
3.1875 0.559666666666667
3.1875 0.654
};
\addplot [thick, dimgray86, forget plot]
table {%
3.15625 0.0921666666666667
3.21875 0.0921666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
3.15625 0.654
3.21875 0.654
};
\addplot [thick, dimgray86, forget plot]
table {%
4.1875 0.454416666666667
4.1875 0.278833333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
4.1875 1.80166666666667
4.1875 2.58
};
\addplot [thick, dimgray86, forget plot]
table {%
4.15625 0.278833333333333
4.21875 0.278833333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
4.15625 2.58
4.21875 2.58
};
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:-0.25,0.0868333333333333)
--(axis cs:-0.125,0.0868333333333333)
--(axis cs:-0.125,0.2115)
--(axis cs:-0.25,0.2115)
--(axis cs:-0.25,0.0868333333333333)
--cycle;
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:0.75,0.147583333333333)
--(axis cs:0.875,0.147583333333333)
--(axis cs:0.875,0.272583333333333)
--(axis cs:0.75,0.272583333333333)
--(axis cs:0.75,0.147583333333333)
--cycle;
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:1.75,0.127833333333333)
--(axis cs:1.875,0.127833333333333)
--(axis cs:1.875,0.334583333333333)
--(axis cs:1.75,0.334583333333333)
--(axis cs:1.75,0.127833333333333)
--cycle;
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:2.75,0.31325)
--(axis cs:2.875,0.31325)
--(axis cs:2.875,0.869)
--(axis cs:2.75,0.869)
--(axis cs:2.75,0.31325)
--cycle;
\path [draw=dimgray86, fill=lavender233232240, thick]
(axis cs:3.75,0.35675)
--(axis cs:3.875,0.35675)
--(axis cs:3.875,0.869833333333333)
--(axis cs:3.75,0.869833333333333)
--(axis cs:3.75,0.35675)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:-0.125,0.0768333333333333)
--(axis cs:0,0.0768333333333333)
--(axis cs:0,0.266083333333333)
--(axis cs:-0.125,0.266083333333333)
--(axis cs:-0.125,0.0768333333333333)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:0.875,0.126)
--(axis cs:1,0.126)
--(axis cs:1,0.265166666666667)
--(axis cs:0.875,0.265166666666667)
--(axis cs:0.875,0.126)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:1.875,0.120083333333333)
--(axis cs:2,0.120083333333333)
--(axis cs:2,0.3015)
--(axis cs:1.875,0.3015)
--(axis cs:1.875,0.120083333333333)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:2.875,0.297)
--(axis cs:3,0.297)
--(axis cs:3,0.640333333333333)
--(axis cs:2.875,0.640333333333333)
--(axis cs:2.875,0.297)
--cycle;
\path [draw=dimgray86, fill=lightgray201201221, thick]
(axis cs:3.875,0.403916666666667)
--(axis cs:4,0.403916666666667)
--(axis cs:4,1.15016666666667)
--(axis cs:3.875,1.15016666666667)
--(axis cs:3.875,0.403916666666667)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:0,0.0659166666666667)
--(axis cs:0.125,0.0659166666666667)
--(axis cs:0.125,0.218666666666667)
--(axis cs:0,0.218666666666667)
--(axis cs:0,0.0659166666666667)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:1,0.107333333333333)
--(axis cs:1.125,0.107333333333333)
--(axis cs:1.125,0.225)
--(axis cs:1,0.225)
--(axis cs:1,0.107333333333333)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:2,0.148)
--(axis cs:2.125,0.148)
--(axis cs:2.125,0.311416666666667)
--(axis cs:2,0.311416666666667)
--(axis cs:2,0.148)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:3,0.24525)
--(axis cs:3.125,0.24525)
--(axis cs:3.125,0.5255)
--(axis cs:3,0.5255)
--(axis cs:3,0.24525)
--cycle;
\path [draw=dimgray86, fill=darkgray162159194, thick]
(axis cs:4,0.47625)
--(axis cs:4.125,0.47625)
--(axis cs:4.125,2.01225)
--(axis cs:4,2.01225)
--(axis cs:4,0.47625)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:0.125,0.0585)
--(axis cs:0.25,0.0585)
--(axis cs:0.25,0.225)
--(axis cs:0.125,0.225)
--(axis cs:0.125,0.0585)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:1.125,0.0981666666666667)
--(axis cs:1.25,0.0981666666666667)
--(axis cs:1.25,0.191083333333333)
--(axis cs:1.125,0.191083333333333)
--(axis cs:1.125,0.0981666666666667)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:2.125,0.146916666666667)
--(axis cs:2.25,0.146916666666667)
--(axis cs:2.25,0.306916666666667)
--(axis cs:2.125,0.306916666666667)
--(axis cs:2.125,0.146916666666667)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:3.125,0.240083333333333)
--(axis cs:3.25,0.240083333333333)
--(axis cs:3.25,0.559666666666667)
--(axis cs:3.125,0.559666666666667)
--(axis cs:3.125,0.240083333333333)
--cycle;
\path [draw=dimgray86, fill=lightslategray126118169, thick]
(axis cs:4.125,0.454416666666667)
--(axis cs:4.25,0.454416666666667)
--(axis cs:4.25,1.80166666666667)
--(axis cs:4.125,1.80166666666667)
--(axis cs:4.125,0.454416666666667)
--cycle;
\addplot [thick, dimgray86, forget plot]
table {%
-0.25 0.0968333333333333
-0.125 0.0968333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
0.75 0.195666666666667
0.875 0.195666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
1.75 0.217666666666667
1.875 0.217666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
2.75 0.399
2.875 0.399
};
\addplot [thick, dimgray86, forget plot]
table {%
3.75 0.5065
3.875 0.5065
};
\addplot [thick, dimgray86, forget plot]
table {%
-0.125 0.0983333333333333
0 0.0983333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
0.875 0.203833333333333
1 0.203833333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
1.875 0.224
2 0.224
};
\addplot [thick, dimgray86, forget plot]
table {%
2.875 0.4595
3 0.4595
};
\addplot [thick, dimgray86, forget plot]
table {%
3.875 0.725666666666667
4 0.725666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
0 0.0956666666666667
0.125 0.0956666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
1 0.161666666666667
1.125 0.161666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
2 0.165833333333333
2.125 0.165833333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
3 0.306333333333333
3.125 0.306333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
4 1.0615
4.125 1.0615
};
\addplot [thick, dimgray86, forget plot]
table {%
0.125 0.0903333333333333
0.25 0.0903333333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
1.125 0.158666666666667
1.25 0.158666666666667
};
\addplot [thick, dimgray86, forget plot]
table {%
2.125 0.188833333333333
2.25 0.188833333333333
};
\addplot [thick, dimgray86, forget plot]
table {%
3.125 0.3445
3.25 0.3445
};
\addplot [thick, dimgray86, forget plot]
table {%
4.125 0.829666666666667
4.25 0.829666666666667
};
\end{axis}

\end{tikzpicture}


==> figures/experiments/math_comparison/relative_total_delay_reduction_congestion_LC.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkslategray63}{RGB}{63,63,63}
\definecolor{peru22412844}{RGB}{224,128,44}
\definecolor{steelblue49115161}{RGB}{49,115,161}

\begin{axis}[
width=\MathComparisonWidth,
height=\MathComparisonHeight,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={[\%]},
xmajorgrids,
xmin=0, xmax=104,
xtick style={color=black},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=1.5,
ytick style={color=black},
ytick={0,1},
yticklabels={$\mathrm{\SigmaUp}$,$\mathrm{\SigmaDown}$}
]


\path [draw=darkslategray63, fill=steelblue49115161]
(axis cs:50.8292382555944,-0.4)
--(axis cs:50.8292382555944,0)
--(axis cs:57.3459075122858,0)
--(axis cs:57.3459075122858,-0.4)
--(axis cs:50.8292382555944,-0.4)
--cycle;
\addplot [darkslategray63]
table {%
50.8292382555944 -0.2
44.1646039534625 -0.2
};
\addplot [darkslategray63]
table {%
57.3459075122858 -0.2
64.2327111826292 -0.2
};
\addplot [darkslategray63]
table {%
44.1646039534625 -0.3
44.1646039534625 -0.1
};
\addplot [darkslategray63]
table {%
64.2327111826292 -0.3
64.2327111826292 -0.1
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0,draw=darkslategray63}, only marks]
table {%
29.3768494678855 -0.2
75.5264207319978 -0.2
81.0262054927472 -0.2
67.3125060137677 -0.2
};
\path [draw=darkslategray63, fill=steelblue49115161]
(axis cs:54.7279310768375,0.6)
--(axis cs:54.7279310768375,1)
--(axis cs:68.7485275735213,1)
--(axis cs:68.7485275735213,0.6)
--(axis cs:54.7279310768375,0.6)
--cycle;
\addplot [darkslategray63]
table {%
54.7279310768375 0.8
44.430257088649 0.8
};
\addplot [darkslategray63]
table {%
68.7485275735213 0.8
79.7227952505371 0.8
};
\addplot [darkslategray63]
table {%
44.430257088649 0.7
44.430257088649 0.9
};
\addplot [darkslategray63]
table {%
79.7227952505371 0.7
79.7227952505371 0.9
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0,draw=darkslategray63}, only marks]
table {%
24.0737949370964 0.8
29.4937797660868 0.8
98.7149356150832 0.8
100 0.8
};
\path [draw=darkslategray63, fill=peru22412844]
(axis cs:80.7506440632672,5.55111512312578e-17)
--(axis cs:80.7506440632672,0.4)
--(axis cs:84.849461766543,0.4)
--(axis cs:84.849461766543,5.55111512312578e-17)
--(axis cs:80.7506440632672,5.55111512312578e-17)
--cycle;
\addplot [darkslategray63]
table {%
80.7506440632672 0.2
76.7370823121396 0.2
};
\addplot [darkslategray63]
table {%
84.849461766543 0.2
86.582270286251 0.2
};
\addplot [darkslategray63]
table {%
76.7370823121396 0.1
76.7370823121396 0.3
};
\addplot [darkslategray63]
table {%
86.582270286251 0.1
86.582270286251 0.3
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0,draw=darkslategray63}, only marks]
table {%
91.6700503049707 0.2
};
\path [draw=darkslategray63, fill=peru22412844]
(axis cs:77.77260805321,1)
--(axis cs:77.77260805321,1.4)
--(axis cs:83.295739589938,1.4)
--(axis cs:83.295739589938,1)
--(axis cs:77.77260805321,1)
--cycle;
\addplot [darkslategray63]
table {%
77.77260805321 1.2
72.6707500546231 1.2
};
\addplot [darkslategray63]
table {%
83.295739589938 1.2
88.6275811060001 1.2
};
\addplot [darkslategray63]
table {%
72.6707500546231 1.1
72.6707500546231 1.3
};
\addplot [darkslategray63]
table {%
88.6275811060001 1.1
88.6275811060001 1.3
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0,draw=darkslategray63}, only marks]
table {%
96.3143601559272 1.2
96.3143601559272 1.2
};
\addplot [darkslategray63]
table {%
53.9625921649586 -0.4
53.9625921649586 0
};
\addplot [darkslategray63]
table {%
59.6071671671917 0.6
59.6071671671917 1
};
\addplot [darkslategray63]
table {%
83.4610363580631 5.55111512312578e-17
83.4610363580631 0.4
};
\addplot [darkslategray63]
table {%
80.8266429247448 1
80.8266429247448 1.4
};
\end{axis}

\end{tikzpicture}

